Variational method for locating invariant tori

We formulate a variational fictitious-time flow which drives an initial guess torus to a torus invariant under given dynamics. The method is general and applies in principle to continuous time flows and discrete time maps in arbitrary dimension, and to both Hamiltonian and dissipative systems.

==> defsTori.tex <==
% defsTori.tex

% Predrag                               Jul 12 2005

    \usepackage[psamsfonts]{amsfonts,amssymb}
    \usepackage{bm}
    \usepackage{graphicx}
    \usepackage[dvips]{color} % dvips allows for colors

        \ifdraft
        \else
    \usepackage[pdfmark,colorlinks]{hyperref} %% hyperlinks
    % \usepackage[pdfauthor={Y. Lan'}%
    %           pdftitle={Invariant Tori},%
    %           pdfmark,colorlinks]{hyperref} %% hyperlinks
    %\usepackage[backref]{hyperref}
        \fi

%%%%%%%%%%%%%%%%%%%%%% COMMENTS %%%%%%%%%%%%%%%%%%%
\ifdraft
  \newcommand{\PC}[1]{{\color{blue} \footnotesize [{\bf PC}: #1]}}
  \newcommand{\CC}[1]{{\color{green}\footnotesize [{\bf CC}: #1]}}
  \newcommand{\YL}[1]{{\color{red}  \footnotesize [{\bf YL}: #1]}}
  \newcommand{\PCedit}[1]{{\color{blue}#1}}
  \newcommand{\CCedit}[1]{{\color{green}#1}}
  \newcommand{\YLedit}[1]{{\color{red}#1}}
\else
  \newcommand{\PC}[1]{}
  \newcommand{\CC}[1]{}
  \newcommand{\YL}[1]{}
  \newcommand{\PCedit}[1]{#1}
  \newcommand{\CCedit}[1]{#1}
  \newcommand{\YLedit}[1]{#1}
\fi
%%%%%%%%%%%%%%%%%%%%%% COMMENTS END %%%%%%%%%%%%%%%

\newcommand{\mpArc}[1]{
           {\tt \href{http://www.ma.utexas.edu/mp_arc-bin/mpa?yn=#1}
           {\goodbreak mp\_arc~#1}}}
\newcommand{\arXiv}[1]{{\tt \href{http://arXiv.org/abs/#1}
           {\goodbreak #1}}}


==> flotsam.tex <==
% flotsam.tex, temporary stuff for tori.tex
% Predrag					Jul 10 2005


\PC{update literature with SIAM DS'05 refs:
\cite{delaLlave04-348,WysMeis05} 
}

\PC{
``In this case we impose the {\em phase condition}'':
\\
remove  (ref {eq:nonsp}) below, and all references to
 {\em non-spiraling condition}. Find definition of the ``phase condition'' in
Frank Schilder, Osinga, Vogt (Bristol) papers
      }

\YL{June 3 2005:\\
The return time (one Poincare map) is $24.18 \pm 0.3$.
	}
\PC{
Is there an unstable periodic orbit in the center? It's complex
eigenvalue should give you the winding rate around the torus.
It should be fairly simple - for the initial guess loop, the points are
obtained by center-of-mass average of each one of your loops as you go
around the torus, and the guess period is  24.2.

Looks like you are looking at a torus created by two successive Hopf
bifurcations, close to onset of chaos in the second limit cycle.
Generically you expect this torus to lock into a mode-locked periodic
orbit, as you increase the parameter (here, slowly increase the size of
the system).
	}

\YL{June 3 2005:\\
 I saw
 chaotic-like motion when increasing the parameter value and found long periodic
 orbit when lowering the parameter.

 I use all the representative points and iterate them once, calculate
 the Jacobian and largest Lyapunov exponent $\lambda$ and do the average. I
 found that $\lambda=0.0080$.

  For many points, two of the eigenvalues(comlex pair) are close
  to one and others are smaller than 1. For a smaller portion of points, one
  eigenvalue is greater than one and others are smaller than 1.

  Take the first representative point and iterate for 
  $t=3032, \lambda=0.0013$,
  the next two exponents being negative and close to zero, 
  others being negative.
  
  when take $t=453.67, \lambda=0.0036$ (??)

 The torus might be weakly repelling or attracting (algebraically?).
 Numerically, it seems that orbit for long stay around the torus but not
 exactly on.
	}

\PC{
 That is what I was worried about - the mere fact that you see it in a time
 series implies that it is nearly attractive. If we could find a partially
 hyperbolic torus, with a strong unstable eigenvalue, it would be more
 impressive.
	}

\PC{

The dimensionless length parameter for KS:
\[
  \tilde{L}=\frac{L}{2 \pi \sqrt{\nu}}   \,.
\]
Spatial wavelength estimated from maximal instability
of the $u=0$ equilibrium, in units of $\tilde{L}$:
\[
  \langle\lambda\rangle = \sqrt{2}   \,.
\]
Previous periodic orbit searches:
\\
 chaotic dynamics  -
 Christiansen, Cvitanovi\'c, and Putkaradze:
  $\tilde{L} \approx 2.889$
  %L = 18.155/(4*a(1)*2)
  %L=18.155 % 1/2 by symetry, of
  %         L=36.31 % \mbox{ or } L=36.30$ % $\nu=1\,,
  % converted from  $\nu=0.029910$, $\nu=0.029924$,
  \\
 chaotic dynamics  -
  Zoldi and Greenside:
  % fixed boundary conditions
  $\tilde{L} \approx 7.958$
  % L=50
  \\
 chaotic dynamics  -
 Lan and Cvitanovi\'c:
  $\tilde{L} \approx 3.0637$ %
  % $L=19.25$ %, $\nu = 1$
  % halved, by symmetry, from $L=38.5$ %, $\nu = 1$

Here, we determine an attracting limit (Hopf) cycle at:
 $\tilde{L}=3.259$
 % $L=20.475$ %, $\nu = 1$
 % halved, by symmetry, from  $L=40.95$ %, $\nu = 1$
This Hopf cycle arises by bifurcation from the stable equilibrium
at $\tilde{L}=3.???$.
\PC{
 Lan, please fill in this parameter value if you know it - perhaps
one of the Frisch et al. solutions.
   }

An attracting limit cycle is usually easy to observe, providing the
trajectory is started in its basin of attraction. So why test the method
on an attracting limit cycle? This is a test of the method where we can
compare it the result of the search with a known target invariant torus.
We would have preferred to test the method on a partially hyperbolic
invariant torus (which, being repelling, cannot be found by running a
typical trajectory forward in time), but that is still out of reach.
   \\
   }
\YL{
 I disagree. Torus of Fig.~\ref{f:ks412a} is a partially hyperbolic
invariant torus, not an attracting limit cycle. I demonstrate this by
computing the linearized stability eigenvalues of the torus (in the full
space, not Poincar\'e section):
 \\
$\Lambda_1 = ?? > 1$,
$\Lambda_{2,3} = e^{\pm \theta_1}$,
$\theta_1 \to$ our $\omega$,
$|\Lambda_k| < 1$ for $k=4,5,\dots$.
   }



\PC{Lan, 

``the torus on
the Poincar\'{e} section $a_1=0.06$. We take $L=40.95$ as our numerical
experiments suggest that an invariant torus exists at this value.''
is presumably a Hopf limit cycle, probably attractive. Can you find
the unstable periodic orbit at its center that it was created from?
	}

\YL{
We used Simo's method~\cite{Simo90}
to compute the unstable manifold on the Poincar\'e section.
It is in our unpublished draft on KSe.

The method of Ref.~\cite{CasJorb00}
is quite similar to ours. The differences are:
\\
1. They cannot determine the shift $\omega$ if it is unknown.
\\
2. They don't have a variational formulation thus don't use the 'Newton's
descent flow'. They solve a big set of nonlinear algebraic equations
\\
3. As a result, their method is not as stable as ours and very good initial
conditions have to be provided in order to converge. The homotopy continuation
is also more complicated.
\\
4. It is hard to change the parametrization.
    } %end \YL{


\PC{
cite %\bibitem{Dieci??} 
?. Dieci,?
}

\PC{references to the ``phase condition'' in
Frank Schilder, Osinga, Vogt (Bristol) papers

to de la Llave, etc...
      }

% Two equivalent approaches exist which lead to the same equation: either
% through a variational technique as in Ref.~\cite{CvitLanCrete02}, or by
% the Newton-Raphson method as in Ref.~\cite{lanVar1}. Here, the first
% method will be adopted for its simplicity.

  
\CC{ Drop: Frequency map analysis 
is a powerful method for
detecting nearly integrable invariant tori  for Hamiltonian systems.}
 % The method utilizes the main frequencies of families of trajectories
 % labeled by initial conditions. 
 %  The
 % variation of these frequencies as a function the initial conditions 
 % leads to a determination of 
 % the existence or not of . 
\CC{Drop: The method is in principle applicable to systems with arbitrary dimension
since it relies on the ability to integrate a large set of trajectories
for a sufficiently long time.}
 % Along these lines several methods have been designed using the time
 % series analysis
 % of integrated trajectories~\cite{f}.  

\CC{Drop: In principle the method is applicable to searches for
$m$-dimensional invariants of maps and 
flows embedded phase spaces of  arbitrary dimension.}

%The summations in Eqs.~(\ref{eq:torreal1})-(\ref{eq:torreal2}) become
%\begin{eqnarray}
%&&\sum_l \left(J_{k-l}^{(r)}
%\frac{d {\bf a}_{l}^{(r)}}{d\tau}-J_{k-l}^{(i)}\frac{d {\bf a}_{l}^{(i)}}{d\tau}\right)= \sum_{l=0}^{k}\left(J_{k-l}^{(r)}\frac{d{\bf a}_{l}^{(r)}}{d\tau}-J_{k-l}^{(i)}\frac{d{\bf a}_{l}^{(i)}}{d\tau}\right) \nonumber \\
%&& \qquad \qquad \qquad
%+\sum_{l=1}^{M-k}\left(J_{l+k}^{(r)}\frac{d{\bf a}_{l}^{(r)}}{d\tau}+J_{l+k}^{(i)}\frac{d{\bf a}_{l}^{(i)}}{d\tau}
%+J_{l}^{(r)}\frac{d{\bf a}_{l+k}^{(r)}}{d\tau}+J_{l}^{(i)}\frac{d{\bf a}_{l+k}^{(i)}}{d\tau}\right), \label{eq:frsum1} \\
%&& \sum_l \left( J_{k-l}^{(r)}
%\frac{d{\bf a}_{l}^{(i)}}{d\tau}+J_{k-l}^{(i)}\frac{d{\bf a}_{l}^{(r)}}{d\tau}\right)= \sum_{l=0}^{k}\left(J_{k-l}^{(i)}\frac{d{\bf a}_{l}^{(r)}}{d\tau}+J_{k-l}^{(r)}\frac{da_{l}^{(i)}}{d\tau}\right)\nonumber \\
%&& \qquad \qquad \qquad
%+\sum_{l=1}^{M-k}\left(J_{l+k}^{(i)}\frac{d{\bf a}_{l}^{(r)}}{d\tau}-J_{l+k}^{(r)}\frac{d{\bf a}_{l}^{(i)}}{d\tau}
%-J_{l}^{(i)}\frac{d{\bf a}_{l+k}^{(r)}}{d\tau}+J_{l}^{(r)}\frac{d{\bf a}_{l+k}^{(i)}}{d\tau}\right)
%. \label{eq:frsum2}
%\end{eqnarray}
 \CC{Drop: From (\ref{eq:torfr}), we solve ${\bf a}_{k}^{(r)}(\tau)$ and ${\bf
a}_{k}^{(i)}(\tau)$ for $k=0,1,\ldots,M-1$. Note that in
(\ref{eq:torfr}), the number of unknowns are one more than the number
of equations.}

 %we have
 %\begin{eqnarray}
 %&&\frac{d_{\bf a}{k}^{(r)}}{d\tau }\cos k\omega-\frac{d {\bf 
 % a}_{k}^{(i)}}{d\tau}\sin k\omega-\sum_l \left(J_{k-l}^{(r)}
 %\frac{d {\bf a}_{l}^{(r)}}{d\tau}-J_{k-l}^{(i)}\frac{d {\bf 
 %a}_{l}^{(i)}}{d\tau}\right) \nonumber \\
%&& \qquad -k\left({\bf a}_{k}^{(r)}\sin k\omega
%+{\bf a}_{k}^{(i)}\cos k\omega \right)\frac{d\omega}{d\tau} =  {\bf b}_{k}^{(r)}-
%{\bf a}_{k}^{(r)}\cos k\omega+{\bf a}_{k}^{(i)}\sin k\omega \label{eq:torreal1} \\
%&&\frac{d{\bf a}_{k}^{(r)}}{d\tau}\sin k\omega+\frac{d{\bf a}_{k}^{(i)}}{d\tau}\cos k\omega-\sum_l \left( J_{k-l}^{(r)}
%\frac{d{\bf a}_{l}^{(i)}}{d\tau}+J_{k-l}^{(i)}\frac{d{\bf a}_{l}^{(r)}}{d\tau}\right)\nonumber \\
%&& \qquad +k\left({\bf a}_{k}^{(r)}\cos k\omega
%-{\bf a}_{k}^{(i)}\sin k\omega \right)\frac{d\omega}{d\tau} =  {\bf b}_{k}^{(i)}-
%{\bf a}_{k}^{(r)}\sin k\omega-{\bf a}_{k}^{(i)}\cos k\omega 
%\,. \label{eq:torreal2}
%\end{eqnarray}


